Investigating VTubing as a Reconstruction of Streamer Self-Presentation: Identity, Performance, and Gender

VTubers, or Virtual YouTubers, are live streamers who create streaming content using animated 2D or 3D virtual avatars. In recent years, there has been a significant increase in the number of VTuber creators and viewers across the globe. This practise has drawn research attention into topics such as viewers' engagement behaviors and perceptions, however, as animated avatars offer more identity and performance flexibility than traditional live streaming where one uses their own body, little research has focused on how this flexibility influences how creators present themselves. This research thus seeks to fill this gap by presenting results from a qualitative study of 16 Chinese-speaking VTubers' streaming practices. The data revealed that the virtual avatars that were used while live streaming afforded creators opportunities to present themselves using inflated presentations and resulted in inclusive interactions with viewers. The results also unveiled the inflated, and often sexualized, gender expressions of VTubers while they were situated in misogynistic environments. The socio-technical facets of VTubing were found to potentially reduce sexual harassment and sexism, whilst also raising self-objectification concerns.

==> tmp.tex <==
%% ----------------------------------------------我是分割線----------------------------------------------

%% Kaiyuan
\subsection{Exaggeration in avatar-mediated performance}

\subsubsection{Existence of exaggerated performance}
Our interviews and observations found that most VTubers (V1-V13) perform exaggeratedly, which tends to be a phenomenon of their self-driven presentation. After the discussion, we divided their exaggerations into three aspects: make exaggerated facial expressions (V5, V11), change to dramatic voice (V3, V8, V12, V13), and perform overacted and contrasted behaviours (V2, V4, V6, V7, V9, V10).
\begin{enumerate}
    \item Make exaggerated facial expressions.
    % \paragraph{Make exaggerated facial expressions}
We found that VTubers exaggerated their facial expressions to present the emotions and energise the atmosphere. V5 stated that she elaborated her facial designs in Live2D based on fans' feedback. When she was making the game streaming,  she could make different facial expressions to interact with the fans emotionally, such as crying, laughing, and annoying. When asking about the difference of using the virtual avatar, she said,

\begin{quote}
In the past, when you played games without showing your face, you could only express emotions through words, but now it can be helped by the facial expressions of virtual avatars. At the same time, avatar is also an appropriate embodiment to express emotions for shy streamers.
\end{quote}
Meanwhile, V11 believed that VTubers should make exaggerated facial expressions to present their feelings, and fans would be more likely to receive emotional signals and participate better in the interactions. 

    \item Change to dramatic voice.
    % \paragraph{Change to dramatic voice}
Instead of making facial expressions, we found it was quite common for VTubers to demonstrate avatars’ personalities with a specialised voice and provide the viewers with a more immersive experience. During the interviews, V12 claimed that 
\begin{quote}
It is straightforward for a real-person live streamer to amplify the emotions by recording. Nevertheless, the facial emotions are relatively monotonous for virtual avatars, so we must use our voice to strengthen the performance (through screaming and voice volume).
\end{quote}
VTubers would utilise the superiority of the voice to express their feelings behind the virtual avatars. In this case, V12 thought that different voices should be used to enhance her emotion, including risen pitch, deepen tone, and louder voice. V13 also reported that,
\begin{quote}
Based on the feedback from my fans, it is my reassuring voice but not the appearance that attracted them. 
\end{quote}
% same quote in section 4.6
According to our observations, multiple features were combined to form the identity of the virtual avatar, which means some VTubers have multifaceted characteristics. We discovered that, as the Nakonohitos behind the avatar, VTubers adjusted their tone, pitch, speed, and other voice attributes to match the characteristics for better performance. For instance, V3 adopted the high-pitched female voice, much sharper and cuter than usual. V8 used some seductive voice to improve the atmosphere and sense of engagement in his audio streaming. His deeper tone was utterly different from the usual voice, which is exaggerated for entertainment requirements. 

    \item Perform overacted and contrasted behaviours.
% \paragraph{Perform overacted and contrasted behaviours}    
Unlike the real-person streamers, the behaviours of VTubers were also found to be overacted and contrasted. According to our observations, it was quite common for VTubers to have dramatic performances. For instance, V2’s identity was a careless girl who would like to play video games, and she spoke many controversial and offensive words without covering up. After observing her fans’ feedback, we found that speaking offensive words was her way to strengthen her personality traits and express her opinions for some breaking news, which made a strong contrast between her cute appearance with the careless identity. V4 claimed that she had multiple personalities and presented different exaggerated behaviours. Her first personality used to be a naughty girl who loved screaming, swearing, and making porn jokes with fans. Another personality is to chat frankly and gently with fans as their true friend. The multifaceted and contrasted behaviours reflect the unique attribute of virtual live streaming, which means that VTubers commonly have diversified and exaggerated performances. 

Similarly, according to our observation, V9 acted like an idiot. He used to swear and make porn jokes with audiences. His fans sent him memes for fun and tended to become idiots like him.  His rude behaviours differed from his cute appearance, which portrayed a contrasted image and strengthened his casual, careless, and humorous personality. In contrast, V6 claimed to have extremely fast calculating speed, so that they could learn fast, store all information, and search quickly. The novel non-human settings brought V6 more flexibility to act exaggeratedly, including changing her height immediately and searching information in an intense short time.
\end{enumerate}


\subsubsection{Motivation and Impact}
% motivation
During the interviews, we found that exaggerated presentation was caused by their limited performance technologically and financially.

When asking about the design and improvement of the avatar without considering technological and financial constraints, most VTubers (V3, V8, V11, V12, V14) desired to have a 3D model. Since the 2D model has performing limitations, for instance, the movements and facial expressions cannot be accurately conveyed without precise recognition. The exaggerations helped in smoothing the recognition process, as mentioned by V11, 
\begin{quote}
Only VTubers’ upper body could be shown in the 2D environment, which typically includes the head and hands movements, so we should make our facial expressions and movements more exaggerated.
\end{quote}
Meanwhile, 2D models impose constraints on video content production; most themes are chatting, gaming, and singing. V8 and V12 thought that the operations of the 2D model are inconvenient and limit the streaming contents, environment and avatar appearance. V3 also mentioned,
\begin{quote}
I would like to have a 3D model to make more exciting genres, such as using the 3D character to make the VLogs…
\end{quote}
However, the financial problem is still a challenge in reality. The 2D model is still regarded as the best tool to present the avatar. While it has obvious limitation, it motivates the exaggerated presentations and became a unique attribute of VTubers. 

% impact
After the discussion, we concluded that exaggerations as a robust approach for VTubers to manage their identity and express themselves.

Virtual avatars have various characteristics, and we discovered that most VTubers try to manage and operate their performance to present a distinctive identity. For instance, V3 reported that 
\begin{quote}
I raised my voice to fit the identity of a young girl. Although not all fans like the raised voice, I think it would be more suitable for an energetic girl, so I insisted on using it.
\end{quote}
Moreover, V8 used a more seductive voice to make the audience enjoy the female-oriented audio streaming immersively. He also used this identity to attract more fans and cater to market needs. V4, V7, and V9 made exaggerated behaviours such as making offensive chats and porn jokes to enhance their careless characteristics and manage their identities. Moreover, V10 performed exaggeratedly to fit her identity as a youngster, using some naughty behaviours and voices.

On the contrary, half of the VTubers (V2, V5, V6, V11 - V14) in our study focused more on using the virtual appearance of the avatar to express their feelings and opinions better. In our interview, V5 told us,
\begin{quote}
My fans’ requirements about the contents were relatively loose, so it mainly depended on my preferences. And my live streaming is more likely to be a place for outputting my personal opinions and interacting with fans emotionally.
\end{quote}
Likewise, V11, V12, and V13 all stated that their virtual avatars had similar personalities with themselves. They intended to adopt some exaggerations to express their views by enhancing some specific characteristics, rather than catering to identity settings. V13 particularly mentioned that she even did not have a setting, and she simply enjoyed using the avatar to present her real feelings. 
Moreover, we observed that V2 and V6 always output their opinions in the live streaming. They used some exaggerated performance to magnify some character traits for more acceptable self-expression and idea demonstration, further connecting with fans more emotionally and immersively providing a more interactive experience.




%% ----------------------------------------------我是分割線----------------------------------------------

%% Christie
\subsection{GENDER LANDSCAPE}
In order to gain further insight into the communication of VTubing, gender demographic demonstrates how individuals represent themselves to others, how others interpret them, and how the interactions create a reciprocal yet exaggerated gender ideology. In other words, the male-to-female ratio in viewers and creators reflect the sociology of gender dominance in the market; the virtual identities develop upon the femininity and masculinity. The demographics of viewers and creators provide the groundwork to illustrate how the creators were treated differently. Through comparing the behaviours and performances between the observed VTubers and perceived gender roles, we reached a consensus on virtual identity bringing a hyper-personal communication by fitting typical gender traits excessively. 

Before delving into the findings, we summarised the traditional gender role portrayals from prior sociology-related studies \cite{Bressler2006, Ford2013, Pilgun2020, Weisberg2011}. The typical lexical description of masculinity refers to the active, ambitious, assertive, authoritative, energetic, and confident leader; whereas femininity is often tied to young, high agreeableness, elegant, sentimental and talkative. Swami et al. \cite{Swami2010} also suggest ideal women images as those who laugh at men's jokes. Men prefer women who have positive personality traits like openness, kindness, and assertiveness, regardless of physical attractiveness. These gender differences are also pervasive in the VTubing field and are elaborated in our findings.

\subsubsection{Demographic and Dominance}
By January in 2022, Virtual YouTuber Wiki, a website storing existing VTuber information (n=1,887), stated that there was 79.1\% female; 19.7\% male; 18 non-binary and 4 gender-fluid virtual streamers. This reveals the prevalence of the creators on the market and shows more female creators than males in this sector. Whereas not every VTubers can provide the gender ratio of their viewers, several participants alluded to the viewers’ demographics. V5, V6 and V13 mentioned most of their viewers were young males respectively. V5 further elaborated there were only 4 girls in her 156 fans chat group. She quoted her friend, a male gaming VTuber, "most of his audiences were male." V11 and V12 provided an estimation of 80\% male viewers. Nevertheless, V8 who is a male VTuber on YouTube stated that 85\% of his viewers were female from YouTube official statistics. We concluded the VTubing industry has a larger male viewers group since it is developed upon Japanese anime, comics, and gaming (ACG) culture. Another significant observation was based on the relationship between the subscribers and the creators according to their genders. V12 depicted the current VTuber market as 
\begin{quote}
...to be a VTuber is more difficult than a YouTuber, and to be a male VTuber is even more difficult than a female VTuber.
\end{quote}
V13 also believed that the male viewers might be attracted by female creators. Supported by the heteronormativity, the statistic underlined the female creators have a greater market share, where is mostly formed by male viewers. Overall, we described the creators as a female-dominated group while viewers as male-dominated fanatics. 
% Not sure if the word patriarchy and matriarchy can be used here.

\subsubsection{Visual Design and Gender Ideology}
We observed that creators strategically develop and edit self-presentation to enable an optimized presentation of avatars. The designed virtual identity is formed from intrinsic characteristics and is further reinforced by their extrinsic features. Here we defined extrinsic features as appearances and outlooks including faces, hair, clothing, and sound. These elements develop the preliminary impression of the characters, influencing how the viewers interact with the creators to form intimacy. We found the design is closely related to gender ideology as it matches typical gender roles in society. The selective identities are self-motivated based on creators’ willingness.
\begin{enumerate}
\item Physical Appearance.
We concluded high agreeableness is highlighted by the presentation form of avatars. 90\% of our female participants are in humanoid non-human images including animals, robotics, and even plants. Male VTubers also tend to include animalistic-related elements in their extrinsic designs. We found an aggregate of pets, humanoid non-human images, and animal incarnations in their design. 

Physical appearances further recognise the characters. We first came to facial outlooks when viewing avatars. All participants were found to have different and unusual eyes colour. We also concluded the common ground of visual designs including big round eyes, double eyelids, small noses, pink blushes and mouths on white skins. In contrast to female VTubers who have round eyes and faces, male VTubers have comparatively longer and masculine facial features such as single eyelids, sharp faces and eyes. Hairstyle is another direct feature showing how avatars are presented. Most participants have special hair colours varying from pink, orange, khaki, pale purple, silver regardless of their gender. V8 also marked the highlights on his hair as his remarkable signature. Still, we found cuteness is being emphasised by the hairstyle of female avatars such as the double tails and buns. In view of the body figure of the characters, V5 described her virtual image as 'a ten-headed body'. While the portrayals of female characters are mainly thin and tall, the male VTubers are also tall yet more muscular via our observations.
%grammar up till here -commonality
Likewise, all participants are dressed and groomed in ways that are stereotypical of their gender. V3 described her summer outfit: 
\begin{quote}
I designed my own dress and you can see (showing her camisole dress), a lot of the lovely animal cartoons (a symbol of V3) is printed on it.
\end{quote}
%V13 also stressed her use of colour in character design in showing her femininity: 
%\begin{quote}
%As my setting is a tender girl, my selection of colour and drawings of avatar is all about creating a gentle feel. That is, many parts and accessories on my body use soft colours such as faint purple and white, to let viewers feel my meek quality.
%\end{quote}
%We observed that the majority of female virtual designs are dressed provocatively and scantily clad. Camisole dresses, cheongsam, plunge dresses are commonly found on females while hoodies, suits are often found on male designs. Such commonalities on visual designs obviously match the beauty standard in society according to gender norms, hence, they are exaggerated as they are not common in reality. 

\item Sound and Voice.
Sound is another formative extrinsic feature in character design. We found that most female streamers tended to be in a higher pitch; whereas male streamers acted to be in lower and desirable tones. A key observation was their voices in our interviews varied their voices in videos and streams. V3 demonstrated the changing of her voice during our interview and said 
\begin{quote}
Higher pitch of the voice is to act cuter, and somehow, more matching on my skin (virtual image as a young girl).
\end{quote}
V12 also shared her idea on voice acting as a female VTuber. She recalled that voice and sound is the direct presentation to viewers: 
\begin{quote}
As a VTuber with a healing and tender setting, it is important for me to strengthen my behaviour and performance with my voice
\end{quote}
%same as ky abt voice
In addition, V13 cited the feedback related to her voice from her viewers that her voice sounds reassuring for them. By the same token on male VTubers, V8 mentioned his changing voice in our interview:
\begin{quote}
Most of the time I will be energetic but I usually turn into a deeper and sexier voice when my fans ask me to
\end{quote}
In sum, we concluded that sounding accentuated the gender features of VTuber: girls are supposedly cute when boys are assumed to be either energetic or sexually sedate.
\end{enumerate}

\subsubsection{Intrinsic Traits and Reinforcements in Virtual Identity}
The first glance of the virtual characters’ visual design provides the preliminary impression but the personality traits pave for uniqueness and form comprehensive virtual identities. Intrinsic attributes refer to how the virtual identity is presented and how the creators perform or behave the characters’ personalities to viewers. 

Female VTubers are usually matching the ideal women images. Most female participants (6 out of 10) are optimistic characters according to their self-proclamation. Specifically, V1, V3, V6 proclaimed themselves as healing influencers, that they aimed to perform gently with positive energy. V5 described herself as “an image of a lively and cheerful big sister” and V12 related her intrinsic features from the point of her audiences’ view: 
\begin{quote}
They like me as a gentle and kind friend. A lot of my viewers reveal their first impression of me as a tender girl and that is the reason why my audiences love to chat with me (the virtual character) from the bottom of their hearts.
\end{quote}
In our observation, V1 strengthened her bonding with audiences by adding interactive components in the presentation to show her kind personality. For example, she put an animated video of a real hand on the head of her virtual image to tap and pet the avatar. Sense of sympathy and adoring is highlighted in her delicate and cheerful image. In spite of positivity, we found several participants (V6, V11) are tough and talkative. They depicted themselves as mannish girls that are androgynous. In our observation on V2 and V4, they were typically friendly, vigorous, casual. They loved to tease one another, even in swear words. Furthermore, V5 further suggested another intrinsic characteristic that was not captured among our participants. She hypothesized a presence of personality highlighting sexiness and female seductiveness. 

Unlike the variety of characteristics found in the female group, we described the male creators as comparatively monotonous. We found the male creators (V7-V10) were all humorous according to the viewers’ perception and their virtual settings. Participants acted idiotic in the stream by telling dirty jokes and memes. For example, V7 was full of male confidence and used mansplaining strategies in his videos which highlighted his masculinity. V8 also said he was a casual, careless, confident, childish, talkative and friendly youngster. These further spot our stereotype of popular males as positive and outgoing. To sum up, these non-realistic yet cordial settings create friendly impressions and build a foundation for the exaggerated behaviour of virtual avatars. In the existing VTubing industry, we found more diversified feminine characters’ traits and monotonous masculine personalities in the designs of virtual identities.

\subsubsection{Gender Sociology in Virtual Community}
During the interview, several interviewees commented that they were treated differently with and without the avatars. V5 recalled her memories as a real video game streamer. She said there was less sexual harassment when having the avatar. She portrayed the live stream using a virtual character as a more harmonious environment comparatively as it effectively reduced mansplainers and the male gaze in chat. V14 also commented virtual avatars were preventing the acquisition of sex viewership. Viewers can no longer build the hierarchical system according to appearance. She recaptured an experience: 
\begin{quote}
And what I felt most deeply was the differences between real and virtual streamers. The female streamer received a gift of 520 yuan. She put the refill directly on her chest and then waved it out towards her viewers. But if it is in my case (under the avatar), all I can do is to say thank you. 
\end {quote}
Several interviewees (V3, V5, V8) preferred the use of avatar than real persona to reduce the criticism from viewers on creators’ appearance. V11 also suggested virtual avatars saved the hassle of makeup. This reduced mansplainers in video game live streaming compared to her experience as a streamer without avatars. These indicate the virtual identity provides a less flirtatious streaming environment for creators on sexual and appearance considerations. 

%% Conclusion （I think this may not be appropriate in finding section? Not sure......)

Overall, the extrinsic features fit the corresponding intrinsic elements in the characters settings to form an attractive character. As physical attractiveness implies positive personality traits, stereotypes about gender personality seem to be largely shared among viewers on creators. The typical gender norms on feminine and masculine affect the exaggerated designs and behaviours of our participants’ virtual identities. The heterosexuality theory further empowers a female-dominated environment for creators by male-dominated fanatics. Therefore, the use of virtual identity offers a comfortable social environment. While the traditional live stream emphasises the differentiation of gender, virtual identity obviously offers perspectives across male and female -  extrinsic and intrinsic aspects of the virtual identity suit the gender norms and how we categorise inherently according to gender; yet achieve gender-blind by neutralising the gender differences in access to and control over resources.



%% ----------------------------------------------------------------------------------------------
\subsection{A customised identity between virtual and real (modified)}
% add example V15 in this section
% V15: topic is history and recordings 記錄 (he)
We found that the identity created by VTubers tend to be mixed between the virtual and their real self, and that to what degree it is virtual or real is customisable. As previously mentioned, many VTubers in our study made up background stories that illustrated their identity in an often virtual world. The identity of V1 and V12, for example, used to be animal that were kept as pet at their home in reality according to their self-proclamation. V5's identity was said to be a plant which is capable of curing all diseases, because she was not in good health condition in real life. Some of the VTubers specifically performed the made-up identity during live streaming as expected in the virtual setting. For instance, V3 claimed her identity be a 14-year-old girl and therefore raised her voice pitch, and sometimes acted cute or naive. V7 \& V10 were said to be teenage boys roughly in high school and we observed they often acted naughty by yelling. 

While we concluded the participants with their customised identities above, the remaining participants emphasised staying true to their own during streams. As an example, V11 said that,
\begin{quote}
    Actually I did not deliberately perform the virtual identity. On the contrary, I run the identity with my personalities in reality. I hope my viewers like my real self rather than just the avatar alone.
\end{quote}
However, many others during our interview study emphasised that their identity during streaming generally stayed true to themselves. As an example, V11 said that,
\begin{quote}
    Actually I did not deliberately perform the virtual identity. On the contrary, I run the identity with my personalities in reality. I hope my viewers like my real self rather than just the avatar alone.
\end{quote}
V13 did not create a background story of her avatar. She explained during interview that,
\begin{quote}
    When streaming as a VTuber, I would not craft a very complicated identity. Perhaps to my mind, it is (just) used for conveying what I want to (stream).
\end{quote}
She later elaborated that she liked to sing behind the avatar. She preferred fans focusing on her singing and the messages conveying behind, to the avatar itself. Others (e.g., V5 \& V12) might be careful in creating their virtual identities, but the way of performing it was said to stayed close to their real selves. V2 was also observed to be voiced normally as speaking in reality. During our interview, V15 said he is self-motivated to decide the themes in his videos, rather than considering viewers' preferences.

Through observation, we also found it was common for VTubers to perform their virtual identities while conveying their opinions on real-life events, and telling personal anecdotes or life experiences. For example, V2 commented on social issues in a non-serious and joking manner during her game streaming; V4 told her personal stories in her chatting sessions to inspire and comfort her viewers; V6 introduced trending news seriously with her personal opinions. 

Regardless of how virtual or how real the identity is, the motivation of customisation was mostly said to be self-driven according to our interviews. For example, V3 said she created a 14-year-old identity simply because she liked it. V8 however, was the only one that claimed his way of performance (especially during some audio streaming) partly market-driven. 

%% ----------------------------------------------我是分割線----------------------------------------------

\subsection{avatar-mediated live streaming practices (modified)}
We observed live streaming practices of a VTuber to be avatar-centred and participatory. It means creators tend to present the streaming and engage with viewers by performing his or her made-up identity, and the streaming usually involves more viewer participation.

%%Notes for amendments
% (solved) this paragraph aims to stress VTuber 直播形象基於人設
% (solved) 特別的顔色應用,i.e. V13 的顔色運用
% (solved) this paragraph aims to stress VTuber 直播内容基於人設
%% (solved) MYA 是一隻畫家的pet, 她表達對主人的不滿和對人類不理解是很正常的
%% (solved) V4 and V5 perform gently 因爲她們的人設
% (solved) this paragraph aims to stress VTuber 在社交平臺用自己的形象來進行直播或交流
%% (solved) 用自己形象visual design to post on the social media platform (image) 預告，收到贊美時也會以形象來多謝
%% (solved) 表情sticker (their avatars) (V1-V4, V6, V8,-V12)
% (keep)this paragraph aims to stress VTuber 本來身份跟 VTubing 或 直播 相關
% (solved) this paragraph aims to stress VTuber viewer participation in 直播内容
%% (solved) 所有particpants 都有雜談向的直播，而雜談上就很多viewer participant 的内容，包括心事台(a platform to let viewers share their expression and let off steam). 
%% (solved) 同人（doujin）refers to self-published creative works produced by a group of people who share an interest, activity, or hobby.\
% (solved) 畫畫、用google map 直播
% this paragraph aims to stress VTuber viewer 更關注有參與度的内容
%观众是因为主播本身才来看直播的 V11V5
\subsubsection{avatar-centred streaming practices}
We found that the live streaming practices of a VTuber were mainly centred around his or her virtual identity. Before the so-called 'debut', a VTuber needs to carefully craft his or her identity, which usually includes the visual design and background of the avatar, and its intended personalities during performance. In other words, their virtual identity provide specific background such as social status, occupations, intended personalities, and V1, V4, V7 even designed working experiences. This further affects the performance in streaming. After the debut, VTubers intended to put on extra seasonal visual design that fit their virtual identities. For example, we observed V1 and V12 changed into a Christmas-style outfit during live streaming on Christmas Eve; V3 mentioned she put on summer clothes because she would like to change clothes along with her fans during summer, which received quite positive feedback. V13 also stressed her use of colour in character design in showing her gentleness: 
\begin{quote}
As my setting is a tender girl, my selection of colour and drawings of avatar is all about creating a gentle feel. That is, many parts and accessories on my body use soft colours such as faint purple and white, to let viewers feel my meek quality.
\end{quote}
Besides, creators might also fine-tune their identities in the way of performing. V3 claimed to have deliberately raised her pitch of voice in order to be a young school girl. Several participants (V7, V11), however, reflected that a virtual identity based on reality was an adaptive performing method. V11 explained that she acted more naturally and closer to herself than the first week of streaming because she found 'being not true to yourself is exhaustive'. 

VTubers' streaming were also found to be presented by performing their virtual identities. The virtual avatar would usually appear in front of the video stream, animated and voiced by the Nakanohito as if it was presented by the real person. We observed the contents develop according to their designed avatars' identity. For instance, V1 depicted herself as a pet who loved to tease her master. Therefore, a lot of her videos involved this content as a joke. V6 also claimed themselves as robotics that controlled by computers, so we found the characters in videos were presented as fast responsive machines. In addition, V4 claimed to have Multiple Personality Disorder in her character setting. She spoke gently during chatting and remained considerate by consoling her fans when they were down, while often swore and screamed wildly during game streaming for fun. These demonstrate avatar-based content design in VTubing.

Furthermore, VTubers tend to build online communities, and actively engage with viewers in the community using their virtual identities. Most of the VTubers (V1, V3-4, V6, V8-9, V11-13) in our study have created a QQ\footnote{https://en.wikipedia.org/wiki/Tencent\_QQ} or Discord group to engage with their fans. Meanwhile, we found that majority of the them (V1-V4, V6, V8-V12) had stickers and memes of their avatar, which can be used in streaming and group chatting. Many of them (V1-4, V8-12) also maintain social media accounts and share their daily life with fans on Twitter, Weibo, Instagram, Facebook, etc. V1 and V3 usually posted their weekly schedule, replied fans' comments, and shared selfies using their virtual avatars. We also observed the common practice among VTubers (e.g., V3 \& V4) of addressing their fans using unique names (such as feathers, people, etc.) that were made up usually before the debut. Besides, some VTubers (e.g., V4 \& V9) were even found to sell merchandise made out of their avatars.

According to our interviews, the motivations of streaming as a VTuber in most cases were found to be a mere attempt at the very beginning. Many of our interviewees used to be a streamer or CG designer, and would like to try VTuber as a fresh start or part-time job. V11 used to have streaming experience, and explained her avatar-centred practices as following:
\begin{quote}
    Due to the presence of the avatar, I will try to create some dramatic effects with it. I used to focus more on the game (during game streaming) than performing (before being a VTuber), and my viewers wouldn't find anything funny with me besides the game.
\end{quote}

\subsubsection{participatory live streaming}
We found the streaming content of a VTuber tend to involve more viewer participation. All VTubers in our study streamed chatting with viewers on a regular basis, such as sharing their expression and letting off steam. Specifically, V1 shared lunch photos with fans; V4 had her fans share their troubles; V9 and V11 browsed through meme videos submitted by his fans. Besides chatting, VTubers would also consider viewer participation when streaming singing, drawing, gaming, etc. For example, V12 made decisions on what a character would look like based on viewer feedback during drawing streams; V1 and V13 sometimes made their viewers order what they would sing during singing streams; V4 invited her fans to play games with her when streaming; V6 commented on her fan-made creative works (\emph{donjin} in Japanese) in her streaming. We also observed creative streaming activities among VTubers (riddle guessing, live poll, finding web pages without searching, Vlogging via Google Map etc.), that were mainly participated by live viewers.

During their interviews, V3 and V11 mentioned that their fans were most likely to be attracted by topics with more participation. This implies to some extent a relatively close relationship are found in between. V5 particularly said the design of her avatar, such as dressing or accessories, were partly determined in discussion with her fans. V8 said he asked the preference from his fans for the topic in his audio streaming, and organised polls on Discord. When asked the most impressive viewer feedback (or interaction), V5 recalled one of her streaming experiences. She accidentally fell asleep in the stream, and her fans tried to contact her friends for her safety. To assure her security, they even started Shiritori using IRC chat in order to show they were always around. V13 also said, 
\begin{quote}
    I had a live stream without prior notice on my birthday. Unexpectedly, I received a re-creation video of my fans in which they sang a song together for me. I was really moved at the moment.
\end{quote}
V11 also mentioned her fans edited collections of videos edition with key features in her streams for recommending potential viewers. V12 recalled that,
\begin{quote}
    I used to have an audience with cancer. He used to watch my streaming during treatment before he passed away. He passed a message via another viewer to me that thanked me for making him happy. His parents also joined my streaming the other day and I conveyed my condolences.
\end{quote}
